Solitonic fermions in the confining phase of SU(2) Yang-Mills theory

We consider spatial coarse-graining in statistical ensembles of non-selfintersecting and one-fold selfintersecting center-vortex loops as they emerge in the confining phase of SU(2) Yang-Mills thermodynamics. This coarse-graining is due to a noisy environment and described by a curve shrinking flow of center-vortex loops locally embedded in a two-dimensional flat plane. The renormalization-group flow of an effective `action', which is defined in purely geometric terms, is driven by the curve shrinking evolution. In the case of non-selfintersecting center-vortex loops, we observe critical behavior of the effective `action' as soon as the center-vortex loops vanish from the spectrum of the confining phase due to curve shrinking. This suggest the existence of an asymptotic mass gap. An entirely unexpected behavior in the ensemble of one-fold selfintersecting center-vortex loops is connected with the spontaneous emergence of order. We speculate that the physics of planar, one-fold selfintersecting center-vortex loops to be relevant for two-dimensional systems exhibiting high-temperature superconductivity.

==> Zusammenfassung.tex <==

\chapter*{Zusammenfassung}
\selectlanguage{german} \pagestyle{plain}

Die wichtigsten Quantenfeldtheorien zur Beschreibung der
Elementarteilchenphysik sind (lokale) Eichtheorien.  Als klassisches
Beispiel seien die Maxwellschen Gleichungen des Elektromagnetismus
angef\"uhrt.  Hierbei handelt es sich um eine abelsche Eichsymmetrie
welche durch die Eichgruppe U(1) beschrieben wird.  Die
Yang-Mills-Theorie ist die Verallgemeinerung auf die bedeutend
komplexeren, nicht abelschen Eichsymmetrien, deren Bewegungsgleichungen,
die Yang-Mills-Gleichungen, im Gegensatz zu den Maxwellschen Gleichungen
nicht linear sind.  Die Quanten-Yang-Mills-Theorie bildet den Eckpfeiler
des Standardmodells der Elementarteilchen und ihrer Wechselwirkungen,
wird darin jedoch nur - aufgrund ihrer Komplexit\"at - im Rahmen der
St\"orungstheorie behandelt.  Nichtsdestotrotz hat das Standardmodell
eine ganze Reihe bemerkenswerter Ergebnisse und Vorhersagen geliefert,
wie zum Beispiel die asymptotische Freiheit der Quantenchromodynamik im
Limes hoher Energien oder die Existenz flavour\"andernder neutraler
Str\"ome \cite{NeutralCurrents}.  Es gibt jedoch immer noch eine
Vielzahl ungel\"oster mathematischer Probleme und unerkl\"arter
Experimente.  Zum einen w\"aren da der fehlende strenge Beweis einer
L\"ucke im Anregungsspektrum der Yang-Mills-Theorie oder die Erkl\"arung
des Farbconfinement \cite{JaffeWitten}.  Zum Anderen steht die Annahme
einer verschwindenden Neutrino-Ruhemasse im Standardmodell im
Widerspruch zur experimentellen Sachlage (erfolgreiche Suche nach dem
doppelten $\beta$-Zerfall \cite{KKG}, und die Vermessung der
Neutrino-Ruhemasse durch die Untersuchung des Spektrums des einfachen
Tritium-$\beta$-Zerfalls \cite{Lobashev1999,Kraus2005}).  Weiterhin ist
die St\"orungsreihe vierdimensionaler Quantenfeldtheorien
h\"ochstwahrscheinlich nur eine asymptotische Entwicklung.  Da die
St\"orungstheorie eine Entwicklung in Potenzen einer notwendigerweise
kleinen Kopplungskonstanten um den a~priori angenommenen Vakuumzustand
der Theorie ist, versagt sie bei der Beschreibung der Physik starker
Kopplungen und den dazugeh\"origen topologisch nicht trivialen
Vakuumzust\"anden.  Daher ist ein nicht st\"orungstheoretischer Zugang
zu den Eichtheorien angeraten.

Eine reine Yang-Mills-Theorie ist invariant unter lokalen
Eichtransformationen und enth\"alt in der Lagrangedichte nur Terme aus
Eichfeldern.  Es gibt eine ganze Reihe von nicht st\"orungstheoretischen
und topologisch nicht trivialen Feldkonfigurationen.  Unter anderem der
Abrikosov-Nielsen-Olesen-Vortex, der 't Hooft-Polyakov-Monopol oder die
Instantonen.  Die Letzteren sind Feldkonfigurationen welche in der
Euklidischen Raumzeit lokalisiert sind (daher der Name Instanton).  Beim
\"Ubergang zu endlicher Temperatur (Kompaktifizierung der Zeit auf einen
Kreis mit Umfang 1/T) werden diese Konfigurationen Kaloronen genannt,
welche weiterhin nach ihrer Holonomie unterschieden werden.  Anschaulich
gesprochen haben Konfigurationen mit nicht trivialer Holonomie eine
Untersruktur: Kaloronen mit nicht trivialer Holonomie enthalten
magnetische (BPS ges\"attigte) Monopole als Konstituenten.

In \cite{Hofmann2005} wurde ein analytischer und nicht
st\"orungstheoretischer Ansatz zur thermodynamischen Behandlung einer
reinen SU(2)-Yang-Mills-Theorie entwickelt. Dabei ist die Hauptidee, den
topologisch nicht trivialen Sektor einem Prozess zu unterziehen, welcher
die Aufl\"osung des System bis zu einer minimalen L\"ange (proportional
zum Inversem eines Skalarfeldes) vergr\"obert,
Aufl\"osungsvergr\"oberung (coarse-graining) genannt.  Dies hat das
Erscheinen von makroskopischen Skalarfeldern und reinen Eichungen zur
Folge.  Die fundamentale Eichsymmetrie wird aufgrund nicht trivialer
thermischer Grundzust\"ande sukzessive gebrochen, was zum Herausbilden
dreier Phasen f\"uhrt.  Diese sind die dekonfinierte, die
pr\"akonfinierte und die konfinierte Phase.  In dieser Diplomarbeit
werden haupts\"achlich die Anregungen der konfinierten Phase der
SU(2)-Yang-Mills-Thermodynamik behandelt.  Die drei unerwarteten
Eigenschaften dieser Phase sind: Das Verschwinden von Druck und
Energiedichte des Grundzustandes bei einer verschwindenden Temperatur
$T=0$.  Der Hagedorn-\"Ubergang von der pr\"akonfinierten zur
konfinierten Phase. Und als letztes, der Spin-1/2 Charakter der
masselosen und massiven Anregungen der konfinierten Phase.

Die dekonfinierte Phase besteht aus wechselwirkenden Kaloronen und
Antikaloronen und hat negativen Druck.  Die propagierenden Anregungen in
dieser Phase sind - aufgrund der durch das makroskopische, emergente
Skalarfeld gebrochenen SU(2)-Symmetrie - zwei massive und und eine
masselose Eichmode.  In der N\"ahe einer kritischen Temperatur f\"uhrt
das Ansteigen der Holonomie mit abnehmender Temperatur zum Zerfall von
Kaloronen und Antikaloronen in magnetische Monopole und Antimonopole.
Durch paarweises kondensieren dieser Monopole bildet sich der
Grundzustand der pr\"akonfinierten Phase heraus.  Die Anregungen der
pr\"akonfinierten Phase sind propagierende, massive duale Eichmoden.
Diese besitzen eine Masse $m_D$ aufgrund der dynamischen Brechung der
beim dekonfinierten-pr\"akonfinierten Phasen \"ubriggebliebenen dualen
U(1)$_D$-Eichsymmetrie.  Instabile Defekte des Grundzustands der
pr\"akonfinierten Phase sind geschlossene magnetische Flussschl\"auche
mit einem Kerndurchmesser $d$.  F\"ur $d>0$ kollabieren diese sofort
wieder sobald sie erzeugt werden, da der negative Druck $P$ innerhalb
der Vortexschleife kleiner ist als au\ss erhalb.  F\"ur Einzelheiten
siehe Abschnitte \ref{sec:ConPhase} und \ref{sec:MbyC}.  Der Druck in
der magnetischen Phase ist negativ.  Beim nicht thermischen Hagedorn
\"Ubergang zur konfinierten Phase findet eine vollst\"andige Entkopplung
der Eichmoden statt.  Mit dem Zerfall des Grundzustandes der
pr\"akonfinierten Phase in Zentrumsvortexschleifen mit und ohne
Schnittpunkte, divergiert die Masse des dualen Eichfeldes $m_D$ und der
Kerndurchmesser $d$ geht gegen Null.  Da $d$ gegen Null geht, ist der
negative Druck auf den verschwindenden Kern des Vortex begrenzt.  Daher
sind Zentrumsvortexschleifen stabile teilchenartige Anregungen f\"ur
$P=0$.  Diese Solitonen werden durch ihre Zentrumsladung und die Anzahl
ihrer Schnittpunkte klassifiziert.  Die Masse eines Solitons mit $N$
Schnittpunkten ist durch $N\Lambda_C$ gegeben, wobei $\Lambda_C$ die
Yang-Mills-Skala ist.  Topologisch gesehen sind Solitonen mit $N>0$
stabil in der Abwesenheit externer Eichmoden, welche an die in den
Schnittpunkten lokalisierten Ladungen koppeln.  F\"ur Solitonen mit
$N=0$ gibt es dagegen keinen topologischen Grund der zur Stabilit\"at
beitr\"agt.

Eine Zentrumsvortexschleife welche in einer zweidimensionalen Ebene im
flachen Raum (lokal) eingebettet ist, wird im Folgenden als planar
bezeichnet.  Es wird nun eine Situation betrachtet wo das Rauschen einer
Umgebung den ansonsten unendlichen d\"unnen Vortexkern aufweicht und
dadurch eine noch endliche Masse $m_D$ und nicht verschwindenden
Kerndurchmesser $d>0$ induziert.  In diesem Falle ist der Druck lokal
ungleich Null, woraufhin die Vortexschleife zu schrumpfen beginnt.
Dieser Prozess wird durch eine nichtlineare partielle
Differentialgleichung zweiter Ordnung in dem dimensionslosen
Flussparameter $\tau$ beschrieben, welche auch Kurvenschrumpfungsfluss
oder W\"armeleitungsgleichung f\"ur Immersionen genannt wird.  Der
Flussparameter $\tau$ ist hierbei eine Variable, welche die Abnahme des
Aufl\"osungsverm\"ogens beschreibt mit der das System betrachtet wird
und ist eine von der entsprechenden Aufl\"osung $Q$ monoton abh\"angende
Funktion.  Dabei ist die Aufl\"osung $Q$ beispielsweise durch den
Impulstransfer in einem Vertex gegeben.  Im Falle einer isolierten
SU(2)-Theorie besteht die Umgebung aus den Sektoren mit $N>0$.  Ist die
konfinierte Phase der SU(2) dagegen Bestandteil eines System mit
zus\"atzlichen Eichsymmetrien, dann wird ein Teil der Umgebung durch die
Mischung mit den entsprechenden Eichgruppen verursacht.  In jedem Fall
wird der vormals unendlich d\"unne Vortexkern aufgrund der
Wechselwirkung mit der Umgebung aufgeweicht, nachdem die
Zentrumsvortexschleife in einem Prozess bei einer endlichen Aufl\"osung
$Q_0$ erzeugt wurde.  Damit ist der Kerndurchmesser der Vortexschleife
$d>0$ und somit auch die Masse des dualen Eichbosons endlich,
$m_D<\infty$.

Entsprechend dem Zugang in \cite{Hofmann2005} werden
Zentrumsvortexschleifen mit einem einzigen Schnittpunkt als Elektronen
und solche ohne Schnittpunkt als die dazugeh\"origen Neutrinos
interpretiert.  Infolgedessen wird die Yang-Mills-Skala $\Lambda_C$ mit
der Elektronenmasse gleichgesetzt, $\Lambda_C=m_e=511$~keV.  Diese
Interpretation wird durch aktuelle Hochtemperaturplasmaexperimenten
gest\"utzt.  Zum einen lassen sich die beobachteten und bisher nicht
erkl\"arbaren Mikroturbulenzen in Tokamak-Experimenten durch das
Auftreten von Imagin\"arteilen in der asymptotischen Entwicklung des
Drucks (nach einer geeigneten Kopplungskonstanten
$\lambda=\exp(-\Lambda_c/T)$) erkl\"aren, siehe auch Abschnitt
\ref{sec:ConPhase}.  Diese Imagin\"arteile werden mit steigender
Temperatur dominant und verletzen das thermische Gleichgewicht
wodurch dann die Mikroturbulenzen entstehen, siehe auch \cite{YMlow}.
Zum anderen lassen sich unerwartet starke und verz\"ogerte Explosionen
in den $Z$-Pinch-Experimenten der Sandia National Laboratories auf die
mit der Temperatur \"uberexponentiell anwachsende Multiplizit\"at von
Solitonenzust\"anden mit $N$ Schnittpunkten erkl\"aren.  Der Spin-1/2
Charakter der Zentrumsvortexschleifen ist eine Folge der Entartung der
Richtung des magnetischen Flusses, welche in einem externen magnetischen
oder elektrischen Feld aufgehoben wird.  Hierbei ist zu erw\"ahnen, dass
ein in Bezug auf die definierende SU(2)-Eichgruppe magnetisches Objekt
(Feld/Ladung) einem elektrischen Objekt (Feld/Ladung) im Standardmodell
der Teilchenphysik entspricht.

Das Verhalten von $N=0$ und $N=1$ Zentrumsvortexschleifen unter
Aufl\"osungsvergr\"oberung wird nun als ein Wilsonscher
Renomierungsgruppenfluss verstanden, welcher einer effektiven \wirkung
unterliegt.  Die Bezeichnung \wirkung ist etwas irref\"uhrend, da wir
nicht darauf abzielen eine Zeitentwicklung des Systems zu erhalten,
indem wir die Stationarit\"at der Wirkung unter einer Variation der
Kurven fordern.  Es werden aufl\"osungsabh\"angige statistische Ensemble
unter dem Einfluss einer Umgebung, welche durch den Parameter $\sigma$
dargestellt wird, betrachtet.  Das entsprechende Gewichtsfunktional der
Ensemblemitglieder ist durch den Exponenten der \wirkung gegeben und in
rein geometrischen Gr\"o\ss en definiert.  Die
Aufl\"osungsabh\"angigkeit der \wirkung wird wiederum durch den
Kurvenschrumpfungsfluss bestimmt.  Die \wirkung wird in einen konformen
und einen nicht konformen Anteil zerlegt.  Es wird nun die Invarianz der
Zustandssumme eines gegebenen Ensembles von planaren Kurven unter dem
Vergr\"obern der Aufl\"osung gefordert.

W\"ahrend eines endlichen Absenkens des Aufl\"osungsverm\"ogens
schrumpfen sich nicht selbst schneidende Zentrumsvortexschleifen ($N=0$)
aufgrund des Rauschens der Umgebung auf eine Punkt zusammen, wobei die
Kurve asymptotisch gegen einem Kreis konvergiert.  Das bedeutet, dass
von einer endlichen kritischen Aufl\"osung $Q_*$ abw\"arts
Zentrumsvortexschleifen nicht mehr aufzul\"osen sind und damit aus dem
Spektrum der konfinierten Phase der SU(2)-Yang-Mills-Theorie
verschwinden.  Dies hat die Existenz einer asymptotischen L\"ucke im
Anregungsspektrum der konfinierten Phase zur Folge, da
Zentrumsvortexschleifen mit $N>0$ eine endliche Masse besitzen.  Der
\"Ubergang zum konformen Limes verschwindender Kurvenl\"ange weist
kritisches Verhalten auf mit einem Mean-Field-Exponenten (0.5) des
Koeffizienten im nicht konformen Anteil der Wirkung, siehe auch
Abschnitt \ref{sec:0RGI}.  Das Verschwinden des $N=0$ Sektors aus dem
Anregungsspektrum der konfinierten Phase der SU(2) und die Nichtexistenz
der Antiteilchen von $N=0$ Zentrumsvortexschleifen stellt eine im
Standardmodell der Elementarteilchenphysik verbotene Verletzung der
Leptonenzahlerhaltung dar.  Damit wird auch die Vorstellung einer
Neutrino-Ruhemasse obsolet.  Die Masse des Neutrinos ist eine Folge der
St\"orungen der Umgebung in die es eingebettet ist und abh\"angig von
der spezifischen Aufl\"osung unter der das System betrachtet wird.  Die
Tatsache, dass Zentrumsvortexschleifen ohne Schnittpunkt ($N=0$) ihre
eigenen Antiteilchen sind, impliziert die Interpretation des Neutrinos
als Majoranateilchen sind.  Diese Interpretation wird durch die
erfolgreiche Suche nach dem neutrinolosen doppelten $\beta$-Zerfalls
gest\"utzt \cite{KKG}.  Weiterhin steigt die Varianz des mittleren \glq
Massen\grq-Schwerpunktes eines Ensembles von $N=0$
Zentrumsvortexschleife von Null aus an und s\"attigt bei einem endlichen
Wert ab bevor es bei einer kritischen Aufl\"osung $Q_*$ verschwindet.
Diese Verhalten \"ahnelt dem eines freien massiven Punktteilchen in
einer Raumdimension in der Quantenmechanik.

Im $N=1$ Sektor wird ein im Vergleich zum $N=0$ Sektor  unerwartetes
Verhalten beobachtet: Sowie die Aufl\"osung abgesenkt wird f\"allt die
Entropie, von einem endlichen Wert beginnend, auf Null ab.  Gleichzeitig
steigt die Varianz des mittleren Schnittpunkts von Null beginnend auf
einen endlichen Wert und sinkt dann wieder auf Null ab, sowie auch die
Entropie auf Null abf\"allt.  Das bedeutet, dass das Ensemble in einen
Zustand extrem hoher Ordnung \"ubergeht, in dem Sinne, dass nur eine
einzige Kurve den Prozess der Aufl\"osungsvergr\"oberung \"uberlebt.
Dies wird von der $\tau$-Entwicklung der einzelnen Gewichte der
Ensemblemitglieder unter dem Kurvenschrumpfungsfluss best\"atigt.
Zuf\"alligerwiese sind in der Natur ebenfalls Systeme realisiert, die
ein unerwartetes Verhalten aufzeigen und deren Dynamik auf
zweidimensionale Ebenen beschr\"ankt ist. Dieses sind Materialien,
welche zu den unkonventionellen Hochtemperatursupraleitern mit besonders
hohen Sprungtemperaturen z\"ahlen.  Nun ist es nahe liegend, dass die
Physik planarer Zentrumsvortexschleifen relevant sein k\"onnte f\"ur die
Beschreibung solcher zweidimensionaler Systeme.

Im Falle der keramischen Hochtemperatursupraleiter, den sogenannten
Kupraten (auf Kupferoxid basierend), welche starke Wechselwirkungen
zwischen den Elektronen aufweisen die innerhalb der supraleitenden
zweidimensionalen Ebene eingesperrt sind, stelle man sich eine Situation
vor wie sie in Abbildung~\ref{fig:Cuprate} aufgezeigt ist.  Sofern durch
eine geeignete Dotierung eine optimale Abschirmung der an den
Schnittpunkten der Zentrumsvortexschleifen lokalisierten
Elektronenladungen gew\"ahrleistet wird, sodass eine anziehende
Wechselwirkung aufgrund des Amp\`ereschen Gesetzes zwischen den
Zentrumsflussschl\"auchen relevant wird, dann ist ein Anordnung wie in
Abbildung~\ref{fig:Cuprate} denkbar.  Hierbei kachelt das System aus
Zentrumsvortexschleifen die zweidimensionale Ebene aus, woraufhin die
relative Verschiebbarkeit der Schnittpunkte der Zentrumsvortexschleifen
untereinander minimal wird.

Das spontane Auftreten von Ordnung im $N=1$ Sektor steht
m\"oglicherweise in engem Zusammenhang mit der k\"urzlich entdeckten
neue Klasse von Hochtemperatursupraleitern, welche auf zweidimensionalen
Eisenarsenid-Systemen basieren.  Diese weisen keine expliziten, starken
Wechselwirkungen zwischen den Elektronen innerhalb der zweidimensionalen
Eisenarsenid-Schicht auf.  Der verschwindende elektrische Widerstand
h\"angt mit der Beobachtung zusammen, dass die Varianz des
Ensemblemittelwertes des Ortes (Schnittpunkt) der elektrischen Ladung
von einer \emph{endlichen} Aufl\"osung $Q_*$ (Temperatur) abw\"arts
verschwindet.  Hierbei ist der Flussparameter $\tau$ eine monotone
Funktion der Aufl\"osung $Q$ (Temperatur).





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: thesis.tex
%%% End: 

